HoloFed: Environment-Adaptive Positioning via Multi-band Reconfigurable Holographic Surfaces and Federated Learning

Positioning is an essential service for various applications and is expected to be integrated with existing communication infrastructures in 5G and 6G. Though current Wi-Fi and cellular base stations (BSs) can be used to support this integration, the resulting precision is unsatisfactory due to the lack of precise control of the wireless signals. Recently, BSs adopting reconfigurable holographic surfaces (RHSs) have been advocated for positioning as RHSs' large number of antenna elements enable generation of arbitrary and highly-focused signal beam patterns. However, existing designs face two major challenges: i) RHSs only have limited operating bandwidth, and ii) the positioning methods cannot adapt to the diverse environments encountered in practice. To overcome these challenges, we present HoloFed, a system providing high-precision environment-adaptive user positioning services by exploiting multi-band(MB)-RHS and federated learning (FL). For improving the positioning performance, a lower bound on the error variance is obtained and utilized for guiding MB-RHS's digital and analog beamforming design. For better adaptability while preserving privacy, an FL framework is proposed for users to collaboratively train a position estimator, where we exploit the transfer learning technique to handle the lack of position labels of the users. Moreover, a scheduling algorithm for the BS to select which users train the position estimator is designed, jointly considering the convergence and efficiency of FL. Our simulation results confirm that HoloFed achieves a 57% lower positioning error variance compared to a beam-scanning baseline and can effectively adapt to diverse environments.

==> sections/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1.in,clip,height=1.25in,clip,keepaspectratio]{./photos/JHu.pdf}}]{Jingzhi Hu} (Member, IEEE) received the B.S. degree at the School of Electrical Engineering and Computer Science and the Ph.D. degree at the School of Electronics at Peking University, in 2017 and 2022, respectively. 
He is currently a research fellow at School of Computer Science and Engineering, Nanyang Technological University.
His main research interests are machine learning, Wi-Fi sensing systems, and reconfigurable intelligent surface-aided RF sensing techniques for the Internet of Things, and has published papers in prestigious venues such as IEEE Journal on Selected Areas in Communications, Transactions on Wireless Communications, Wireless Communications, and ACM MobiCom.
He served as a TPC Member for IEEE/CIC ICCC in 2017 and 2018.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1.in,clip,height=1.25in,clip,keepaspectratio]{./photos/ZChen.pdf}}]{Zhe Chen} (Member, IEEE) is an assistant professor within the School of Computer Science at Fudan University, and the Co-Founder of AIWiSe Ltd. Inc. He obtained his Ph.D. degree in Computer Science from Fudan University, China, with a 2019 ACM SIGCOMM China Doctoral Dissertation Award. Before joining Fudan University, he worked as a research fellow in NTU for several years, and his research achievements, along with his efforts in launching products based on them, have thus earned him 2021 ACM SIGMOBILE China Rising Star Award recently.
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[width=1.in,clip,height=1.25in,clip,keepaspectratio]{./photos/TZheng.pdf}}]{Tianyue Zheng} (Graduate Student Member, IEEE) is a Ph.D. candidate in Computer Science at Nanyang Technological University, Singapore. He holds a B.Eng. degree in Telecommunication Engineering from Harbin Institute of Technology, China, and an M.Eng. degree in Computer Engineering from the University of Toronto, Canada. His research focuses on RF sensing and deep learning, and he has published papers in prestigious venues such as  IEEE INFOCOM, IEEE Transactions on Mobile Computing, IEEE Communications Magazine, ACM MobiCom, ACM SenSys, and ACM UbiComp.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1.25in,clip,height=1.25in,keepaspectratio]{./photos/RSchober.pdf}}]{Robert Schober} (Fellow, IEEE) received the Diplom (Univ.) and the Ph.D. degrees in electrical engineering from Friedrich-Alexander University of Erlangen-Nuremberg (FAU), Germany, in 1997 and 2000, respectively. From 2002 to 2011, he was a Professor and Canada Research Chair at the University of British Columbia (UBC), Vancouver, Canada. Since January 2012 he is an Alexander von Humboldt Professor and the Chair for Digital Communication at FAU. His research interests fall into the broad areas of Communication Theory, Wireless and Molecular Communications, and Statistical Signal Processing.

Robert received several awards for his work including the 2002 Heinz Maier Leibnitz Award of the German Science Foundation (DFG), the 2004 Innovations Award of the Vodafone Foundation for Research in Mobile Communications, a 2006 UBC Killam Research Prize, a 2007 Wilhelm Friedrich Bessel Research Award of the Alexander von Humboldt Foundation, the 2008 Charles McDowell Award for Excellence in Research from UBC, a 2011 Alexander von Humboldt Professorship, a 2012 NSERC E.W.R. Stacie Fellowship, a 2017 Wireless Communications Recognition Award by the IEEE Wireless Communications Technical Committee, and the 2022 IEEE Vehicular Technology Society Stuart F. Meyer Memorial Award. Furthermore, he received numerous Best Paper Awards for his work including the 2022 ComSoc Stephen O. Rice Prize. Since 2017, he has been listed as a Highly Cited Researcher by the Web of Science. Robert is a Fellow of the Canadian Academy of Engineering, a Fellow of the Engineering Institute of Canada, and a Member of the German National Academy of Science and Engineering.

He served as Editor-in-Chief of the IEEE Transactions on Communications, VP Publications of the IEEE Communication Society (ComSoc), ComSoc Member at Large, and ComSoc Treasurer. Currently, he serves as Senior Editor of the Proceedings of the IEEE and as ComSoc President-Elect.
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[width=1.in,clip,height=1.25in,clip,keepaspectratio]{./photos/JLuo.pdf}}]{Jun Luo} (Senior Member, IEEE) received his BS and MS degrees in Electrical Engineering from Tsinghua University, China, and the Ph.D. degree in Computer Science from EPFL (Swiss Federal Institute of Technology in Lausanne), Lausanne, Switzerland. From 2006 to 2008, he has worked as a postdoctoral research fellow in the Department of Electrical and Computer Engineering, University of Waterloo, Waterloo, Canada. In 2008, he joined the faculty of the School Of Computer Science and Engineering, Nanyang Technological University in Singapore, where he is currently an Associate Professor. His research interests include mobile and pervasive computing, wireless networking, machine learning and computer vision, security and privacy, as well as applied operations research. More information can be found at \url{https://personal.ntu.edu.sg/junluo}.
\end{IEEEbiography}

